The effect of COVID-19 vaccinations on self-reported depression and anxiety during February 2021

Using the COVID-19 Trends and Impact survey, we find that COVID-19 vaccinations reduced the prevalence of self-reported feelings of depression and anxiety, isolation, and worries about health among vaccine-accepting respondents in February 2021 by 3.7, 3.3, and 4.3 percentage points, respectively, with particularly large reductions among respondents aged 18 and 24 years old. We show that interventions targeting social isolation account for 39.1\% of the total effect of COVID-19 vaccinations on depression, while interventions targeting worries about health can account for 8.3\%. This suggests that social isolation is a stronger mediator of the effect of COVID-19 vaccinations on depression than worries about health. We caution that these causal interpretations rely on strong assumptions.

==> tables/fullsampleoutcomebounds.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Wed Sep 29 10:40:10 2021
\begin{table}[ht]
\centering
\caption{Outcome estimates: non-parametric bounds} 
\label{tab:fullsamplebounds1}
\begin{tabular}{lll}
  \hline
Outcome & Estimate & Bounds \\ 
  \hline
Depressed & -4.40 (-5.12, -3.69) & (-15.25, -3.29) \\ 
  Worried about health & -4.34 (-5.53, -3.15) & (-15.62, -2.82) \\ 
  Isolated & -3.72 (-4.34, -3.09) & (-14.56, -2.76) \\ 
   \hline
\end{tabular}
\end{table}


==> tables/mediation-table-five.tex <==
\begin{table}[!h]

\caption{Mediation analysis: GLM estimates, dichotimized mediator (95\% CI) \label{tab:medtab5}}
\centering
\begin{threeparttable}
\begin{tabular}[t]{lllll}
\toprule
Effect & Ref = 0 & Proportion (Ref = 0) & Ref = 1 & Proportion (Ref = 1)\\
\midrule
IDE & -2.27 (-2.50, -2.04) & 60.97 (58.00, 63.95) & -2.36 (-2.60, -2.12) & 63.30 (60.19, 66.41)\\
IIE & -1.45 (-1.56, -1.35) & 39.03 (36.05, 42.00) & -1.37 (-1.38, -1.35) & 36.70 (33.59, 39.81)\\
IIE - Isolated & -1.10 (-1.20, -1.00) & 29.53 (26.94, 32.12) & -1.03 (-1.13, -0.94) & 27.76 (25.10, 30.42)\\
IIE - Health & -0.34 (-0.37, -0.31) & 9.13 (8.19, 10.07) & -0.31 (-0.35, -0.28) & 8.45 (7.38, 9.51)\\
IIE - Covariant & -0.01 (-0.02, 0.00) & 0.36 (0.08, 0.64) & -0.02 (-0.12, 0.09) & 0.50 (0.05, 0.94)\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item IDE represents the interventional direct effect; IIE represents the total interventional indirect effect; IIE - X represents interventional indirect effect via the indicated channel X; Ref represents the reference category for the indirect effects
\end{tablenotes}
\end{threeparttable}
\end{table}


==> tables/mediation-table-four.tex <==
\begin{table}[!h]

\caption{Mediation analysis: missing hesitancy included (95\% CI) \label{tab:medtab4}}
\centering
\begin{threeparttable}
\begin{tabular}[t]{lllll}
\toprule
Effect & Ref = 0 & Proportion (Ref = 0) & Ref = 1 & Proportion (Ref = 1)\\
\midrule
IDE & -1.93 (-2.16, -1.70) & 51.95 (48.50, 55.39) & -2.05 (-2.30, -1.81) & 55.22 (51.42, 59.02)\\
IIE & -1.79 (-1.90, -1.67) & 48.05 (44.61, 51.50) & -1.67 (-1.71, -1.62) & 44.78 (40.98, 48.58)\\
IIE - Isolated & -1.45 (-1.55, -1.34) & 38.87 (35.86, 41.89) & -1.39 (-1.50, -1.28) & 37.38 (34.09, 40.66)\\
IIE - Health & -0.31 (-0.34, -0.27) & 8.21 (7.16, 9.26) & -0.24 (-0.28, -0.19) & 6.39 (5.11, 7.67)\\
IIE - Covariant & -0.04 (-0.06, -0.01) & 0.97 (0.29, 1.65) & -0.04 (-0.16, 0.09) & 1.01 (-0.09, 2.11)\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item IDE represents the interventional direct effect; IIE represents the total interventional indirect effect; IIE - X represents interventional indirect effect via the indicated channel X; Ref represents the reference category for the indirect effects
\end{tablenotes}
\end{threeparttable}
\end{table}


==> tables/mediation-table-three.tex <==
\begin{table}[!h]

\caption{Mediation analysis: GLM estimates, suspicious responses excluded (95\% CI) \label{tab:medtab3}}
\centering
\begin{threeparttable}
\begin{tabular}[t]{lllll}
\toprule
Effect & Ref = 0 & Proportion (Ref = 0) & Ref = 1 & Proportion (Ref = 1)\\
\midrule
IDE & -1.98 (-2.21, -1.75) & 51.99 (48.59, 55.39) & -2.09 (-2.33, -1.84) & 54.77 (51.18, 58.36)\\
IIE & -1.83 (-1.94, -1.71) & 48.01 (44.61, 51.41) & -1.72 (-1.76, -1.68) & 45.23 (41.64, 48.82)\\
IIE - Isolated & -1.50 (-1.61, -1.39) & 39.37 (36.39, 42.34) & -1.43 (-1.54, -1.32) & 37.66 (34.50, 40.82)\\
IIE - Health & -0.30 (-0.34, -0.27) & 8.00 (6.99, 9.00) & -0.24 (-0.28, -0.20) & 6.35 (5.18, 7.53)\\
IIE - Covariant & -0.02 (-0.05, 0.00) & 0.65 (-0.02, 1.32) & -0.05 (-0.17, 0.07) & 1.21 (0.23, 2.19)\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item IDE represents the interventional direct effect; IIE represents the total interventional indirect effect; IIE - X represents interventional indirect effect via the indicated channel X; Ref represents the reference category for the indirect effects
\end{tablenotes}
\end{threeparttable}
\end{table}


==> tables/mediation-table-two.tex <==
\begin{table}[!h]

\caption{Mediation analysis: GLM estimates, hesitant included (95\% CI) \label{tab:medtab2}}
\centering
\begin{threeparttable}
\begin{tabular}[t]{lllll}
\toprule
Effect & Ref = 0 & Proportion (Ref = 0) & Ref = 1 & Proportion (Ref = 1)\\
\midrule
IDE & -2.00 (-2.25, -1.76) & 66.49 (62.43, 70.55) & -1.93 (-2.20, -1.67) & 64.07 (59.14, 69.01)\\
IIE & -1.01 (-1.14, -0.88) & 33.51 (29.45, 37.57) & -1.08 (-1.14, -1.03) & 35.93 (30.99, 40.86)\\
IIE - Isolated & -1.02 (-1.15, -0.90) & 33.97 (30.06, 37.89) & -0.98 (-1.10, -0.85) & 32.36 (28.14, 36.59)\\
IIE - Health & 0.00 (-0.07, 0.07) & -0.03 (-2.46, 2.40) & -0.09 (-0.16, -0.02) & 2.96 (0.73, 5.19)\\
IIE - Covariant & 0.01 (-0.08, 0.10) & -0.44 (-3.40, 2.53) & -0.02 (-0.17, 0.13) & 0.60 (-1.30, 2.51)\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item IDE represents the interventional direct effect; IIE represents the total interventional indirect effect; IIE - X represents interventional indirect effect via the indicated channel X; Ref represents the reference category for the indirect effects
\end{tablenotes}
\end{threeparttable}
\end{table}


==> tables/mnarboundsoutcome-cc.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Wed Sep 29 10:40:08 2021
\begin{table}[ht]
\centering
\caption{Outcome sensitivity: R = 0 confounded} 
\label{tab:marbounds2}
\begin{tabular}{lll}
  \hline
Outcome & CC Estimate & Bounds \\ 
  \hline
Depressed & -3.78 (-4.03, -3.53) & (-17.41, -3.03) \\ 
  Health & -4.18 (-4.48, -3.88) & (-17.80, -3.34) \\ 
  Isolated & -3.43 (-3.70, -3.16) & (-17.12, -2.72) \\ 
   \hline
\end{tabular}
\end{table}


==> tables/mnarboundsoutcome.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Thu Sep 16 11:55:29 2021
\begin{table}[ht]
\centering
\caption{Outcome sensitivity: MNAR bounds} 
\label{tab:marbounds2}
\begin{tabular}{ll}
  \hline
Outcome & MNAR Bounds \\ 
  \hline
Depressed & (-18.22, -2.84) \\ 
  Worried about health & (-18.37, -2.05) \\ 
  Isolated & (-17.95, -2.75) \\ 
   \hline
\end{tabular}
\end{table}


==> tables/modelperformance2.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Mon Feb 21 13:51:30 2022
\begin{table}[ht]
\centering
\caption{Outcome models: predictive performance on observed data (GLM)} 
\label{tab:modelperf2}
\begin{tabular}{lrrrr}
  \hline
Outcome & Balanced Accuracy & Precision & Sensitivity & Specificity \\ 
  \hline
Depressed & 0.56 & 0.59 & 0.14 & 0.98 \\ 
  Health & 0.57 & 0.59 & 0.20 & 0.94 \\ 
  Isolated & 0.52 & 0.55 & 0.05 & 0.99 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/modelperformance3.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Mon Feb 21 13:51:30 2022
\begin{table}[ht]
\centering
\caption{Outcome models: predictive performance on observed data (XGBoost)} 
\label{tab:modelperf3}
\begin{tabular}{lrrrr}
  \hline
Outcome & Balanced Accuracy & Precision & Sensitivity & Specificity \\ 
  \hline
Depressed & 0.56 & 0.56 & 0.16 & 0.97 \\ 
  Health & 0.52 & 0.53 & 0.06 & 0.99 \\ 
  Isolated & 0.57 & 0.59 & 0.19 & 0.95 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/senstab3.tex <==
% latex table generated in R 4.2.0 by xtable 1.8-4 package
% Fri Jan 27 13:43:32 2023
\begin{table}[ht]
\centering
\caption{Estimate sensitivity: alternative complete-case definition} 
\label{tab:senstab3}
\begin{tabular}{lll}
  \hline
Outcome & Primary Estimates & Alternative complete-case \\ 
  \hline
Depressed & -3.72 (-3.98, -3.47) & -3.69 (-3.94, -3.44) \\ 
  Isolated & -3.26 (-3.53, -2.99) & -3.26 (-3.53, -3.00) \\ 
  Worried about health & -4.26 (-4.55, -3.96) & -4.28 (-4.58, -3.99) \\ 
   \hline
\end{tabular}
\end{table}


==> tables/senstab6.tex <==
% latex table generated in R 4.2.0 by xtable 1.8-4 package
% Wed Feb  1 12:24:18 2023
\begin{table}[ht]
\centering
\caption{Estimate sensitivity: non-essential activities 
 (instead of isolation)} 
\label{tab:senstab6}
\begin{tabular}{ll}
  \hline
Outcome & Effects \\ 
  \hline
Depression & -3.65 (-3.91, -3.40) \\ 
  Activities &  2.00 ( 1.66,  2.33) \\ 
  Health & -4.27 (-4.57, -3.97) \\ 
   \hline
\end{tabular}
\end{table}

